Machine Learning for Mechanical Ventilation Control

We consider the problem of controlling an invasive mechanical ventilator for pressure-controlled ventilation: a controller must let air in and out of a sedated patient's lungs according to a trajectory of airway pressures specified by a clinician. Hand-tuned PID controllers and similar variants have comprised the industry standard for decades, yet can behave poorly by over- or under-shooting their target or oscillating rapidly. We consider a data-driven machine learning approach: First, we train a simulator based on data we collect from an artificial lung. Then, we train deep neural network controllers on these simulators.We show that our controllers are able to track target pressure waveforms significantly better than PID controllers. We further show that a learned controller generalizes across lungs with varying characteristics much more readily than PID controllers do.

==> ML4H 2021/1.abstract.tex <==
\begin{abstract}
Mechanical ventilation is one of the most widely used therapies in the ICU. However, despite broad application from anaesthesia to COVID-related life support, many injurious challenges remain.

We frame these as a control problem: ventilators must let air in and out of the patient's lungs according to a prescribed trajectory of airway pressure. Industry-standard controllers, based on the PID method, are neither optimal nor robust.

Our data-driven approach learns to control an invasive ventilator by training on a simulator itself trained on data collected from the ventilator. This method outperforms popular reinforcement learning algorithms and even controls the physical ventilator more accurately and robustly than PID.

These results underscore how effective data-driven methodologies can be for invasive ventilation and suggest that more general forms of ventilation (e.g., non-invasive, adaptive) may also be amenable.


%Mechanical ventilation is one of the most widely used therapies in the ICU, with applications including anaesthesia and life support during the current COVID-19 pandemic. 
%Many challenges remain in mechanical ventilation that can lead to ventilator-induced lung injury for patients, motivating the need for furthur research. We investigate this challenge from the perspective of ventilator control. 

%Specifically, we consider the problem of controlling an invasive mechanical ventilator: a controller must let air in and out of a sedated patient's lungs according to an airway pressure trajectory specified by a clinician. Industry standard controllers are based on the PID method, which is neither optimal nor robust for this application.

%We investigate several reinforcement learning methods, and propose a model-based approach: we train simulators based on data collected from an artificial lung. 
%We then show that neural network-based controllers trained on these simulators outperform other methods, including PID, in terms of tracking accuracy and robustness  on the artificial lung.
%Our trained simulators significantly improve upon previous physics-based simulators, and may be of independent interest. 
%These results show the effectiveness of a data-driven methodology for invasive ventilation, that can potentially be extended to more general forms of ventilation, including non-invasive and adaptive ventilation.


% MOVE TO CONCLUSIONS !!!

%From a scientific perspective, we find the reinforcement learning problem of ventilation has understudied attributes: it allows for differentiation through the environment. Our study demonstrates that for differentiable reinforcement learning problems, the paradigm of simulation and direct policy optimization can outperform general-purpose RL methods in terms of sample and computational complexity. 


%\eh{we also benchmark other RL methods. we find that sim+deep control is best, maybe due to the differentiability.}

%\eh{make a point about simulator data based vs. physics}

%CONCLUSION? From a scientific perspective, we find the reinforcement learning problem of ventilation has understudied attributes: it allows for differentiation through the environment. Our study demonstrates that for differentiable reinforcement learning problems, the paradigm of simulation and direct policy optimization can outperform general-purpose RL methods in terms of sample and computational complexity. 

\end{abstract}



==> ML4H 2021/2.intro.tex <==
\section{Introduction}

%\ds{By the end of intro, the reader should feel we have a medically important \textbf{\textit{and}} RL-interesting problem}



Mechanical ventilation is a widely used treatment with applications spanning anaesthesia \citep{coppola2014protective}, neonatal intensive care \citep{van2019modes}, and life support during the current COVID-19 pandemic \citep{meng2020intubation, wunsch2020mechanical, mohlenkamp2020ventilation}. This life-sustaining treatment has two common modes: invasive ventilation, where the patient is fully sedated, and assist-control ventilation, where the patient can initiate breaths \citep{patientventasynch}. 

Even though mechanical ventilation has been deployed in ICUs for decades, several challenges remain that can lead to ventilator-induced lung injury (VILI) for patients \citep{vili}. In pressure-support ventilation, a form of assist-control ventilation, evidence suggests that a combination of high peak pressure and high tidal volume can lead to tissue injury in the lung \citep{vili_1}. Pressure-support ventilation also suffers from patient-ventilator asynchrony, where the patient's breathing pattern does not match the ventilator's, and can result in hypoxemia (low level of blood oxygen), cardiovascular compromise, and patient discomfort \citep{asynchrony}.

However, the risk of developing VILI depends not only on factors related to the ventilator, but also on intrinsic characteristics of the patient's lung \citep{vili}. These characteristics usually cannot be directly observed, so trained clinicians must continuously monitor the patient. Given the highly manual process of mechanical ventilation, it is desirable to have control methods that can better track prescribed pressure targets and are robust to variations of the patient's lung.

%Paragraph about the importance of developing robust control methods for mechanical ventilators and recent advances in RL are promising directions. 

Motivated by this potential to improve patient health, we focus on pressure-controlled invasive ventilation (PCV) \citep{rittayamai2015pressure} as a starting point. In this setting, an algorithm controls two valves that let air in and out of a patient's lung according to a target waveform of lung pressure (see Figure \ref{fig:tracking}). We consider the control task only on ISO-standard \citep{ISO68844} artificial lungs.

\paragraph{State of the art.} 
Despite its importance, ventilator control has remained largely unchanged for years, relying on PID \citep{pid2} controllers and similar variants to track patient state according to a prescribed target waveform. %The reliance on the tested-and-tried PID method is not unique to medical ventilation - PID is ubiquitous in control of medical systems. 
However, this  approach is not optimal in terms of tracking---PID can overshoot, undershoot, and exhibit ringing behavior for certain lungs. It is also not sufficiently robust---ventilators are carefully tuned during design, manufacture, and maintenance \citep{ziegler1942optimum,chen2012control} and any changes in ventilator dynamics (e.g., tubing, response delay), environment (e.g., atmospheric pressure), or patient must be accounted for and continuously monitored by trained clinicians via various physical controls on the ventilator \citep{rees2006using}. % \ds{Moved safety point further down. we have citations, but we don't address it fully with experiments}


%Paragraph about this work focusing on mechanical ventilation as a proof of concept, since it's more accessible and easier to tackle. 
%Data-driven approaches are promising, clinical trials out of scope


% Invasive mechanical ventilation is a common medical treatment in which a ventilator controls all breathing for a fully-sedated patient and is used in applications spanning anaesthesia \citep{coppola2014protective}, neonatal intensive care \citep{van2019modes}, and life support during the current COVID-19 pandemic \citep{meng2020intubation, wunsch2020mechanical, mohlenkamp2020ventilation}. 

%In this work, we focus on pressure-controlled invasive ventilation (PCV) \citep{rittayamai2015pressure}, a setting in which an algorithm controls two valves that let air in and out of a patient's lung according to a target waveform of lung pressure (see Figure \ref{fig:vent-control-problem}). 
\begin{figure}[!h]
     \centering
     \includegraphics[width=0.5\textwidth]{figures/circuit.pdf}
     \caption{A simplified respiratory circuit showing the airflow through the inspiratory pathway, into and out of the lung, and out the expiratory pathway. We shade the components that our algorithms can control in green.}
     \label{fig:circuit}
 \end{figure}%

 \begin{figure}[!h]
     \centering
     \includegraphics[width=0.45\textwidth]{figures/tracking.pdf}
     \caption{An example run of three breaths where PID (dark gray line) controls lung pressure (blue line) according to a prescribed target waveform (orange line).}
     \label{fig:tracking}
 \end{figure}


\paragraph{Challenges of ventilator control.} 


%partial observation of a complex system, we don't know system parameters, controller needs to quickly adapt. so we build a more expressive model, but that requires tons of data. that requires a simulator. 

A ventilator controller must adapt quickly and reliably across the spectrum of clinical conditions, which are only indirectly observable given a single measurement of pressure. 
A model that is highly expressive may learn the dynamics of the underlying systems more precisely and thus adapt faster to the patient's condition. However, such models usually require a large amount of data to train, which can take prohibitively long to collect by purely running the ventilator. We opt instead to learn a simulator to generate artificial data, though learning such a simulator for a partially observed non-linear system is itself a difficult problem.

%This motivates learning a simulator to generate artificial data. 
%However, learning a simulator for a partially observed nonlinear system is by itself a difficult problem. 

%In general it can be statistically ill-posed: there are unstable policies for which closed-loop dynamics exhibit chaos.

%Learning a reliable simulator is the problem of nonlinear system identification under partial observation, which can be a statistically ill-posed problem in the worst case: there are unstable policies for which the closed-loop dynamics exhibit chaos. \xc{not sure what this means}


%We study a residual approach to the safe exploration of the system's dynamics.

%We also consider the challenge of generalizing across dynamical systems. While the PID controller has few parameters and thus does exhibit some generalization, its performance on lungs with physical characteristics it was not tuned for is in general unsatisfactory, and fine-tuning or manual intervention by a clinician is required. 




\subsection{Our contributions} 

We present better-performing, more robust results and present resources for future researchers. Specifically, 
\begin{enumerate}

    \item We demonstrate that learning a controller as a neural network correction to PID outperforms its uncorrected counterpart (optimality).
    
    \item We show that a single learned controller trained on several ISO lung settings outperforms the PID controller that performs best across the same settings (robustness).
    
    \item We provide self-contained differentiable simulators for the ventilation problem. These simulators  reduce the entrance cost for future researchers to contribute to invasive mechanical ventilation. 
    
    \item We conduct a methodological study of reinforcement learning techniques, both model-based and model-free, including policy gradient, Q-learning and other variants. We conclude that model-based approaches are more sample and computationally efficient. 
    
%    \item  We demonstrate the potential of an end-to-end pipeline for learning a controller, improving upon PID controllers for tracking pressure waveforms. These improvements are measured based upon ISO standards for performance of ventilatory support equipment \citep{ISO68844}.  \xc{echo the optimality point in challenges of ventilator control}
    
    
\end{enumerate}


%We remark that a unique feature of our work is that it is model-based with an actual physical mode. 
%Many recent works in sample-efficient reinforcement learning are concerned with long-term planning under a learned model of the environment's dynamics. Several recent influential works learn a differentiable simulation of a non-differentiable environment that does not involve a hardware setup (like MuJoCo physics, or the rules of chess). Our work learns differentiable simulators from physical data. \xc{not sure what this paragraph is supposed to say?} \eh{me neither... should ask Cyril perhaps}

Of note, we limit our investigation to open-source ventilators. Control methods used by proprietary ventilators cannot be modified or assessed independently from their hardware and such equipment are cost-prohibitive for academic research.

We see this study as a preliminary investigation of machine learning for ventilator control. In future work, we hope to extend this methodology to non-invasive ventilation, pressure-support ventilation, and conduct clinical trials. 

% \subsection{Structure of the paper}
% In the next subsection we discuss related work. In Section \ref{sec:background} we present the background on both control and ventilation physics, as well as out motivation for a model-based approach. We describe our hardware setup for the mechanical ventilator in Section \ref{sec:hardware}. The details on how we learn and evaluate a data-driven differentiable simulator for the mechanical ventilator are provided in Section \ref{sec:sim}. In Section \ref{sec:control} we describe the learning procedure for our controller and report on the end-to-end experimental results. Section \ref{sec:benchmarks} describes a comparison of RL approaches for ventilation.  Additional details on the simulator and controller learning are provided in the Appendix.


\subsection{Related work}\label{sec:related}

The modern positive-pressure ICU mechanical ventilator dates back to the 1940s \citep{kacmarek11} with many open-source ventilator designs \citep{ventlist} published during the COVID-19 pandemic.

Yet at their core, ventilators all rely on controlling air in and out of an elastic lung via a respiratory circuit, as described in many physics-based models \citep{PMID:8420408}. Such simple operation masks the complexity of treatment \citep{chatburn2011closed} and recent work on augmenting PID controllers with adaptive methods \citep{9122946,PPR:PPR169448} have sought to address more advanced clinical needs. To the best of our knowledge, our data-driven approach of learning both simulator and controller is novel in this field.

\paragraph{Control and RL in virtual and physical systems.} Much progress has been made on learning dynamics when the dynamics themselves exist \emph{in silico}: MuJoCo physics \citep{hafner2019learning}, Atari games \citep{kaiser2019model}, and board games \citep{schrittwieser2020mastering}. Combining such data-driven models with either pixel-space or latent-space planning has been shown to be effective  for policy learning. \citep{ha2018recurrent} is an example of this research program for the deep learning era. Progress on deploying end-to-end learned agents (i.e. controllers) in the physical world is more limited in comparison, due to difficulties in scaling parallel data collection and higher variability in real-world data. \citep{bellemare2020autonomous} present a case study on autonomous balloon navigation using a Q-learning approach, rather than a  model-based one like ours. \citep{akkaya2019solving} use domain randomization with non-differentiable simulators for a difficult dexterous manipulation task.

% A manifestation of this research program for the current deep learning era is established in \citep{ha2018recurrent}.

% \paragraph{Control and RL in physical systems.} Progress on deploying end-to-end learned agents (i.e. controllers) in the physical world is more limited in comparison, due to difficulties in scaling parallel data collection and higher variability in real-world data. \citep{bellemare2020autonomous} present a case study on autonomous balloon navigation using a Q-learning approach, rather than a  model-based one like ours. \citep{akkaya2019solving} use domain randomization with non-differentiable simulators for a difficult dexterous manipulation task.

\paragraph{System identification and residual policy learning. } System identification has been studied for decades in control and reinforcement learning,  %, with the linear case well understood \citep{learningwithoutmixing,improper}. 
see e.g. \citep{schoukens2019nonlinear,billings1980identification} for nonlinear system identification.   Deep neural networks have been used to represent nonlinear dynamics, see e.g. \cite{helicopter}. Residual policy learning \citep{rpl} is a model-free analogue of our controller design: it learns a correction term on an initial, imperfect policy, and is shown to be more data-efficient than learning from scratch, especially for complex robotic tasks. More recently, concurrent work by \citep{pidcar} uses residual policy learning to improve PID for the car suspension control problem.
%\ds{ICML reviewers asked about sys id and Residual RL (PID control with RL)}

\paragraph{Multi-task reinforcement learning.} Part of our methodology has close parallels in multi-task reinforcement learning \citep{taylor2009transfer}, where the objective is to learn a policy that performs well across diverse environments. To make our controllers more robust, we optimize our policy simultaneously on an ensemble of learned models corresponding to different physical settings, similar to the work of \citep{rajeswaran2016epopt, chebotar2019closing} on robotic manipulation.

\paragraph{Machine learning for health applications.} Healthcare offers a multitude of opportunities and challenges for machine learning; for a survey, see \citep{ghassemi2020review}. Specifically, reinforcement learning and control have found numerous applications \citep{yu2020reinforcement}, and recently for weaning patients off mechanical ventilators \citep{prasad2017reinforcement,yu2019inverse,yu2020supervised}. As far as we know, there is no prior work on improving the control of ventilators using machine learning. 



==> ML4H 2021/3.background.tex <==


\section{Scientific background}
\label{sec:background}

\subsection{Control of dynamical systems}

We begin with some formalisms of the control problem. A partially-observable discrete-time dynamical system is given by the following equation: 
$$ x_{t+1} = f(x_t, u_t), o_{t+1} = g(x_{t+1})$$
where  $x_t$ is the underlying state of the dynamical system, $o_t$ is the observation of the state available to the controller, $u_t$ is the control input and $f,g$ are the transition function and observation functions respectively. Given a dynamical system, the control problem is to minimize the sum of cost functions over a long-term horizon:
\begin{align*}
& \min_{u_{1:T} }  \sum_{t=1}^T c_t(x_t, u_t) \quad \text{s.t.}\;\; x_{t+1} = f_t(x_t, u_t).
\end{align*}

This problem is in general computationally intractable, and theoretical guarantees are available for special cases of dynamics (notably linear dynamics) and perturbations. For an in-depth exposition on the subject, see the textbooks by \citet{Bertsekas17,kemin,tedrake}. 

\paragraph{PID control.} A ubiquitous technique for the control of dynamical systems is the use of linear error-feedback controllers, i.e. policies that choose a control based on a linear function of the current and past errors vs. a target state. That is,
$$ u_{t+1} = \sum_{i=0}^k \alpha_i \eps_{t-i} , $$
where $\eps_t = x_t - {x}^{\star_t}$ (or $\eps_t = o_t - {o}^{\star_t}$ if the system is partially-observable) is the deviation from the target state at time $t$, and $k$ represents the history length of the controller. PID applies a linear control with \emph{proportional}, \emph{integral}, and \emph{differential} coefficients,
$$ u_t = \alpha \eps_{t} + \beta \sum_{i=0}^k \eps_{t-i} + \gamma (\eps_{t} - \eps_{t-1}) .  $$
This special class of linear error-feedback controllers, motivated by physical laws, is a simple, efficient and widely used technique  \citep{PID1}. It is currently the industry standard for (open-source) ventilator control.  

\subsection{The physics of ventilation}
\label{subsec:physics}
In invasive ventilation, the ventilator is connected to a patient's main airway, and applies pressure in a cyclic manner to simulate healthy breathing. During the inspiratory phase, the target applied pressure increases to the peak inspiratory pressure (PIP). During the expiratory phase, the target decreases to the positive-end expiratory pressure (PEEP), maintained in order to prevent the lungs from collapsing. The PIP and PEEP values, along with the durations of these phases, define the time-varying target \emph{waveform}, specified by the clinician.

% In invasive ventilation, a patient is connected to the ventilator with a hollow tube that goes into their mouth and down into their main airway or trachea. The ventilator is connected to a central pressure chamber, and applies pressure in a cyclic manner to simulate healthy breathing. During the inspiratory phase, the target applied pressure increases to the peak inspiratory pressure (PIP). During the expiratory phase, the target decreases to the positive-end expiratory pressure (PEEP), maintained in order to prevent the lungs from collapsing. The PIP and PEEP values, along with the durations of these phases, define the time-varying target \emph{waveform}, specified by the clinician.

The goal of ventilator control is to regulate the pressure sensor measurements to follow the target waveform $p_t^{\star}$ via controlling the air-flow into the system which forms the control input $u_t$. As a dynamical system, we can denote the underlying state of the ventilator-patient system as $x_t$ evolving as $x_{t+1} = f(x_t, u_t),$ for an unknown $f$ and the pressure sensor measurement $p_t$ is the observation available to us. The cost function can be defined to be a measure of the deviation from the target; e.g. the absolute deviation $c_t(p_t, u_t) = |p_t - p_t^{\star}|$. The objective is to design a controller that minimizes the total cost over $T$ time steps. 

A ventilator needs to take into account the structure of the lung to determine the optimal pressure to induce. Such structural factors include \textit{compliance} ($C$), or the change in lung volume per unit pressure, and \textit{resistance} ($R$), or the change in pressure per unit flow.

\paragraph{Physics-based model.} A simplistic formalization of the ventilator-lung dynamical system can be derived from the physics of a connected two-balloon system, with a \emph{latent state} $v_t$ representing the volume of air inside the lung. The dynamics equations can be written as
$$v_{t+1} = v_t + u_t \cdot \Delta_t$$ $$p_t = p_0 + \left( 1 - \left( \frac{r_t}{r_0} \right)^6 \right) \cdot \frac{1}{r_t r_0^2}, \;\;r_t = \left( \frac{3 v_t}{4 \pi} \right)^{1/3},$$ where $p_t$ is the measured pressure, $v_t$ is volume, $r_t$ is radius of the lung, $u_t$ is the input air flow rate, and $\Delta_t$ is the time increment. $u_t$ originates from a pressure difference between lung-pressure $p_t$ and supply-pressure $p_\text{supply}$, regulated by a valve: $u_t = \frac{p_\text{supply} - p_t}{R_\text{in}}$. The resistance of the valve is $R_\text{in}\propto 1/d^4$ (Poiseuille's law) where $d$, the opening of the valve, is controlled by a motor. The constants $p_0,r_0$ depend on both the lung and ventilator.  In \cite{nadeem_2021}, several physics-based models are benchmarked, showing errors that are an order of magnitude larger than what can be achieved with a data driven approach.  While the interpretability of such models is appealing, their low fidelity is prohibitive for offline reinforcement learning.


\subsection{Challenges and benefits of a model-based approach}

The physics-based dynamics models described above are highly idealized, and are suitable only to provide coarse predictions for the behaviors of very simple controllers. We list some sources of error arising from using physics equations for model-based control:
\begin{itemize}
    \item \emph{Idealization of physics:} oversimplifying fluid flow and turbulence via ideal incompressible gas assumptions; linearizing the dynamics of the lung and ventilator components.
    \item \emph{Lagged and partial observations:} assuming instantaneous changes to volume and pressure across the system. In reality, there are non-negligible propagation times for pressure impulses, delayed pressure feedback arising from lung elasticity, and computational latency.
    \item \emph{Underspecification of variability:} different patients' clinical scenarios, captured by the latent constants $p_0, r_0$, may intrinsically vary in more complex (i.e. higher-dimensional) ways.
\end{itemize}

Due to the reasons listed above, it is highly desirable to adopt a learned model-based approach in this setting because of its sample-efficiency and reusability. A reliable simulator enables much cheaper and faster data collection for training a controller, and allows us to incorporate multitask objectives and domain randomization (e.g. different waveforms, or even different patients). An additional goal is to make the simulator \emph{differentiable}, enabling direct gradient-based policy optimization through the system's dynamics (rather than stochastic estimates thereof).

We show that in this partially-observed (but single-input single-output) system, we can query a reasonable amount of training data in real time from the test lung, and use it offline to learn a differentiable simulator of its dynamics (\emph{``real2sim''}). Then, we complete the pipeline by leveraging interactive access to this simulator to train a controller (\emph{``sim2real''}). We demonstrate that this pipeline is sufficiently robust that the learned controllers can outperform PID controllers tuned directly on the test lung.

==> ML4H 2021/4.experimental.tex <==
\section{Experimental Setup}
\label{sec:hardware}

To develop simulators and control algorithms, we run mechanical ventilation tasks on a physical test lung \citep{ingmar_medical_2020} using the open-source ventilator designed by Princeton University's People's Ventilator Project (PVP) \citep{pvp2020}.

\subsection{Physical test lung}
For our experiments, we use the commercially-available adult test lung, ``QuickLung'', manufactured by IngMar Medical. The lung has three lung compliance settings ($C=\{10, 20, 50\}$ mL/cmH2O) and three airway resistance settings ($R=\{5, 20, 50\}$ cmH2O/L/s) for a total of 9 settings, which are specified by the ISO standard for ventilatory support equipment \citep{ISO68844}. An operator can change the lung's compliance and resistance settings manually. We connect the test lung to the ventilator via a respiratory circuit \citep{canadian1986canadian, parmley1972disposable} as shown in Figure \ref{fig:circuit}. Figure \ref{fig:vent-farm} shows a snapshot of our hardware setup.

% An operator can change the lung's compliance by engaging one or more springs that modify the difficulty of inflating the lung. To change airway resistance, the operator changes the diameter of the inlet to restrict or relax airflow. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=7cm]{figures/vent-farm.jpg}
    \caption{The ventilator cluster we constructed to run our experiments, featuring 10 ventilators, 4 air compressors, and 2 control servers. Each ventilator is re-calibrated after each experimental run for consistency across ventilators and over time.}

    \label{fig:vent-farm}
\end{figure}

\subsection{Mechanical ventilator}
There are many forms of ventilator treatment. In addition to various pressure target trajectories, clinicians may want to focus on other factors, such as volume and flow \citep{chatburn2007classification}. The PVP ventilator focuses on targeting pressure for a completely sedated patient (i.e., the patient does not initiate any breaths) and comprises two pathways (see Figure \ref{fig:circuit}): (1) the inspiratory pathway that regulates airflow into the lung and (2) the expiratory pathway for airflow out of the lung. A software controller is able to adjust one valve for each pathway. The inspiratory valve is a proportional control flow valve that allows control in a continuous range from fully closed to fully open. The expiratory valve is a binary on-off valve that only permits zero or maximum airflow.

To prevent damage to the ventilator and/or injury to the operator, we implement software overrides that abort a given run: 1) if pressure or volume in the lung exceeds certain thresholds, 2) if tubing disconnects, or 3) if there is significant software delay. The PVP pneumatic design also includes a safety valve in case software overrides fail.



% In addition to various target trajectories, clinicians may want to choose the physical quantity being targeted (e.g., volume, flow, or pressure of air), what ends a breath, and whether or not the patient initiates any breaths \citep{chatburn2007classification}.

% The PVP ventilator focuses on targeting pressure for a completely sedated patient (i.e., the patient does not initiate any breaths) and comprises two pathways (see Figure \ref{fig:circuit}): (1) the inspiratory pathway that directs, regulates, and monitors airflow into the lung and (2) the expiratory pathway that does the same for airflow out of the lung. A software controller is able to adjust one valve for each pathway. The inspiratory valve is a proportional control flow valve that allows control in a continuous range from fully closed to fully open. The expiratory valve is a binary on-off valve that only permits zero or maximum airflow.

% To prevent damage to the ventilator and/or injury to the operator, we implement four software overrides that abort a given run by closing the inspiratory valve and opening the expiratory valve: 1) if pressure in the lung exceeds 70 cmH2O, 2) if volume in the lung exceeds 1.2L, 3) if pressure in the lung drops below PEEP (5 cmH2O) for more than 300ms (indicates disconnected tubing), or 4) if we observe that the average sampling period exceeds 40ms over 300ms (indicates software delays). The PVP pneumatic design also includes a safety valve, which lets out air whenever internal pressure is in excess of 1 PSI (70 cmH2O), in case software overrides fail.

\subsection{Abstraction of the simulation task}
We treat the mechanical ventilation task as episodic by separating each inspiratory phase (e.g., light gray regions in Figure \ref{fig:lung-task}) from the breath timeseries and treating those as individual episodes. This approach reflects both physical and medical realities. Mechanically ventilated breaths are by their nature highly regular and feature long expiratory phases (dark gray regions in Figure \ref{fig:lung-task}) that end with the ventilator-lung system close to its initial state, thereby justifying the episodic nature. Further, the inspiratory phase is indeed the most relevant to clinical treatment and the harder regime to control with prevalent problems of under- or over-shooting the target pressure and ringing. Naturally thus, we attempt to learn a simulator for the ventilator-lung dynamics for the inspiratory phase. To this end repeated episodes of inspiratory phases are thus simplified, faithful units of training data.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/lung-task.pdf}
    \caption{PID controllers exhibit their suboptimal behavior (under- or over-shooting, ringing) primarily during the inspiratory phase. Note that we use a hard-coded controller during expiratory phases to ensure safety. This choice does not affect our results.}
    \label{fig:lung-task}
\end{figure}


==> ML4H 2021/5.simulator.tex <==

\section{Learning a data-driven simulator} \label{sec:sim}

With the hardware setup outlined in Section~\ref{sec:hardware}, we have a physical system suitable for benchmarking, in place of a true patient's lung. In this section, we present our approach to learning a simulator for the inspiratory phase of this ventilator-lung system, subject to the practical constraints of real-time data collection. Two main considerations drive our simulator training and evaluation design:  

First, the evaluation for any simulator can only be performed using a {\bf black-box metric}, since we do not have explicit access to the system dynamics, and existing physics models are poor approximations to the empirical behavior. 
    
Second, the dynamical system we simulate is very challenging for a comprehensive simulation covering all modalities and in particular exhibits chaotic behavior in boundary cases. Therefore, since the end goal for the simulator is better control, we only evaluate the simulator for ``reasonable" scenarios that are relevant to the control task.
    %We thus explore within a neighborhood of realistic open loop trajectories.
    



\subsection{Black-box simulator evaluation}\label{sec:sim_metric}

% To evaluate our data-driven simulator for the mechanical ventilation system, we take into consideration that 
% \begin{enumerate}
%     \item Access to the physical system is black-box only and costly in terms of time/compute. That is, we have no explicit approximation of the dynamics equation. 
    
%     \item
%     The simulator dynamics are complex non-linear operations given by a deep neural network. 
% \end{enumerate}
The class of learned simulators we consider are deep neural networks and thus in addition to the lack of explicit access to system dynamics, the simulator dynamics are also complex non-linear operations. Thus we deviate from standard distance metrics (between the simulator and the true system) considered in the literature, such as \citet{ferns2005metrics}, as they explicitly involve the value function over states, transition probabilities or other unknown quantities. Rather, we consider metrics that are based on the evolution of the dynamics, as studied in \citet{vishwanathan2007binet}. 

However, unlike the latter work, we take into account the particular distribution over control sequences that we expect to search around during the controller training phase. We thus define the following distance between dynamical systems.
Let $f_1,f_2$ be two dynamical systems over the same state-action spaces. % $\mathbf{U} \subseteq \reals^{d_u} \ , \  \mathbf{X} \subseteq \reals^{d_x} $.  
Let $\D$ be a distribution over sequences of controls denoted $\mathbf{u} = \{u_1,u_2,...,u_T\}$.
We define the {\bf open-loop distance} w.r.t. horizon $T$ and control sequence distribution $\D$ as
    \begin{align*}
    \|f_1 - f_2\|_{ol} \defeq \E_{\mathbf{u} \sim \D} \left[ \sum_{t=1}^T \| f_1(x_{t,1},u_t) - f_2(x_{t,2},u_t) \|  \right] . \end{align*}
    
    
% \begin{enumerate}
%     \item We let the {\bf open-loop distance} w.r.t. horizon $T$ and control sequence distribution $\D$ be defined as
%     \begin{align*}
%     & \|f_1 - f_2\|_{ol} \equiv \\
%     & \E_{u_{1:T} \sim \D} \left[ \sum_{t=1}^T \| f_1(x_{t,1},u_t) - f_2(x_{t,2},u_t) \|  \right] . \end{align*}
    
%     \item We let the {\bf closed-loop distance} w.r.t. horizon $T$ and policy distribution $\mu$ be defined as
%     \begin{align*}
%     & \|f_1 - f_2\|_{cl} \equiv \\
%     & \E_{\pi \sim \mu} \left[ \sum_{t=1}^T \| f_1(x_{t,1},\pi(x_{t,1})) - f_2(x_{t,2},\pi(x_{t,2})) \| \right] .
%     \end{align*}

% \end{enumerate}
We use the Euclidean norm over the states in the inner loop, although this can be generalized to any metric. Compared to metrics involving feedback from the simulator, the open-loop distance is a more reliable description of transfer, since it minimizes hard-to-analyze interactions between the policy and the simulator.

We evaluate our data-driven simulator using the open loop distance metric, and we illustrate a result in the top half of Figure~\ref{fig:sim_testing}. In the bottom half, we show a sample trajectory of our simulator and the ground truth. See Section \ref{sec:sim_model} for experimental details. 

\begin{figure}
\centering
\includegraphics[width=8cm]{figures/sim-testing.pdf}
\caption{Performance for a learned simulator for ventilator + a particular lung setting $R=5, C=50$. The upper plot shows the \textit{open-loop distance} and the lower shows a sample trajectory with a fixed sequence of controls (open-loop controls), both for lung setting . In the former, we see low error as we increase the number of steps we project and in the latter, we see that our simulated trajectory tracks the true trajectory quite closely.}\label{fig:sim_testing} 
\end{figure}

\subsection{Data-collection via targeted exploration}\label{sec:safe_exp}
Motivated by the black-box metric described above, we focus on collecting trajectories comprising of control sequences and the measured pressure sequences upon the execution of the control sequences to form a training dataset. Due to safety and complexity issues, we cannot hope to exhaustively explore the space of all trajectories. Instead keeping the eventual control task in mind, we choose to explore trajectories \textit{near} the control sequence generated by a baseline PI controller. The goal is to have the simulator faithfully capture the true dynamics in a reasonably large vicinity of the optimal control trajectory on the true system. To this end, for each of the lung settings, we collect data by choosing a safe PID controller baseline and introducing random exploratory perturbations according to the following two policies:
\begin{enumerate}
    \item Boundary exploration: To the very beginning of the inhalation, add an additional control sampled uniformly from $(c^a_{\min}, c^a_{\max})$ and decrease this additive control linearly to zero over a time frame sampled randomly from $(t^a_{\min}, t^a_{\max})$; 
    \item Triangular exploration: sample a maximal additional control from a range $(c^b_{\min}, c^b_{\max})$ and an interval $(t^b_{\min}, t^b_{\max})$, within the inhalation. Start from $0$ additional control at time $t^b_{\min}$, increase the additional control linearly until $(t^b_{\min} + t^b_{\max}))/2$, and then decrease to $0$ linearly until $t^b_{\min}$.
\end{enumerate}

For each breath during data collection, we choose policy $(a)$ with probability $p_a$ and policy $(b)$ with probability $(1-p_a)$. The ranges in $(a)$ and $(b)$ are lung-specific. We give the exact values used in the Appendix.

This protocol balances the need to explore a significant part of the state space with the need to ensure safety. The boundary exploration capitalizes on the fact that at the beginning of the breath, exploration is safer and also more valuable. The former, due to the lung being at steady state and the latter due to the fact that the typical target waveform for inhalation requires a rapid pressure increase with a quick switch to stabilization, leading to a need for better understanding of dynamics in the early phases of a breath. The structure for the triangular exploration is inspired by the need for a persistent exploration strategy (similar ideas exist in \cite{dabney2020temporally}) which can capture intrinsic delay in the system. We illustrate this approach in Figure \ref{fig:exp_data}: control inputs used in our exploration policy are shown on the top, and the pressure measurements of the ventilator-lung system are shown on the bottom. Precise parameters for our exploration policy are listed in Table \ref{table:appendix-sim-data} in the Appendix.

\begin{figure}\centering
\includegraphics[width=8cm]{figures/exploratory.pdf}
\caption{We overlay the controls and pressures from all inspiratory phases in the upper and lower plots, respectively. From this example of the simulator training data (lung setting $R=5, C=50$), we see that we explore a wide range of control inputs (upper plot), but a more limited ``safe'' range around the resulting pressures.}\label{fig:exp_data}
\end{figure}

\subsection{Model architecture}\label{sec:sim_model}

Now we describe the architectural details of our data-driven simulator. Due to the inherent differences across lungs, we opt to learn a different simulator for each of the tasks, which we can wrap into a single meta-simulator through code that selects the appropriate model based on a user's input of $R$ and $C$ parameters.

\paragraph{Training Task(s).} The simulator aims to learn the unknown dynamics of the inhalation phase. We approximate the state of the system (which is not observable to us) by the sequence of the past pressures and controls upto a history length of $H_c$ and $H_p$ respectively. The task of the simulator can now be distilled down to that of predicting the next pressure $p_{t+1}$, based on the past $H_c$ controls $u_{t},\ldots, u_{t-H_c}$ and $H_p$ pressures $p_{t},\ldots, p_{t-H_p}$. We define the training task by constructing a regression data set whose inputs come from contiguous overlapping sections of $H_p, H_c$ within the collected trajectories and the task is to predict the following pressure.

\paragraph{Boundary Model} Towards further improvement of simulator performance we found that, additional distinction needs to be provided for difference in the behavior of the dynamics during the "rise" and "stabilize" phases of an inhalation. Thus we learned a collection of individual models for the very beginning of the inhalation/episode and a general model for the rest of the inhalation, mirroring our choice of exploration policies. This proves to be very helpful as the dynamics at the very beginning of an inhalation are transient, and also extremely important to get right due to downstream effects. Concretely, our final model stitches together a list of $N_B$ boundary models and a general model, whose training tasks are as described earlier (details found in Appendix \ref{app:sim}, Table \ref{table:appendix-sim-training}). 

% \paragraph{Model architecture details} For the general model, we use a $d$ layer self-normalizing neural network \citep{snn}, where each hidden layer has width $W$. Each boundary model is a simple 2-layer feed-forward neural network with $W$ hidden units and $\tanh$ activation. We perform an architecture search across the various architectural parameters $H_p, H_c, W, N_B, d$ and include the results in the Appendix~\ref{app:sim}. In particular for a couple of lung settings, we further include the entire search space to provide an ablation study of what parts of the architecture/featurization are important. 

% \paragraph{Evaluation.} We evaluate our simulators by holding out $10\%$ of data collected according to our exploration protocol described in \ref{sec:safe_exp} and computing the average open-loop distance over the inspiratory phases, as described in \ref{sec:sim_metric}. In Figure \ref{fig:sim_testing}, we see a qualitative representation of our simulator's performance on the $R=5, C=50$ task. The associated score is $-$ average open-loop distance normalized by episode length. We provide further details for the remaining 8 settings in Appendix \ref{app:sim-evaluation}.



==> ML4H 2021/6.controller.tex <==
\section{Learning controllers from learned physics} \label{sec:control}

% \subsection*{TODO}
% \begin{itemize}
%     \item Featurizaton ablation
%     \item With/withoud pid ablation
%     \item architecture search
% \end{itemize}

In this section we describe the following two controller tasks:
\begin{enumerate}
    \item {\bf Performance:} improve performance for tracking desired waveform in ISO-specified benchmarks. Specifically, we minimize the combined $L_1$ deviation from the target inhalation behavior across all target pressures on the simulator corresponding to a single lung setting of interest.
    \item {\bf Robustness:} improve performance using a {\bf single} trained controller. Specifically, we minimize the combined $L_1$ deviation from the target inhalation behavior across all target pressures \textit{and} across the simulators corresponding to \textit{several} lung settings of interest.
\end{enumerate}

\paragraph{Controller architecture.} 
Our controller is comprised of a PID baseline upon which we learn a deep network correction controlled with a regularization parameter $\lambda$. This \textit{residual} setup can be seen as a regularization against the gap between the simulator and the real dynamics. In particular this prevents the controller training from over-fitting on the simulator. We found this approach to be significantly better than the directly using the best (and perhaps over-fitted) controller on the simulator. We provide further details about the architecture and ablation studies in the Appendix. %Hereafter, use this general architecture to construct controllers for both the tracking improvement task and the generalization task. 
% We use this general architecture to construct both lung-specific (\textit{local}) and lung-agnostic (\textit{shared}) final controllers which we ultimately test on the mechanical lung. 

%\paragraph{Baseline PID.} The baseline PID of a controller for the tracking improvement task is set to the most performant PID controller from a grid search on the corresponding physical lung setting\footnote{When a sufficient baseline does not exists, we choose a baseline of $0$.}. The baseline PID of a controller for the generalization task is set to the PID with the lowest average error across all lung settings. We describe more details in Appendix \ref{app:data-best-pid} and Table \ref{table:appendix-best-pid}.

% ELAD: I removed this... imo not neded
%This approach is naturally applicable to practical scenarios, since existing ventilators are deployed in conjunction with a controller. \pg{don't know how to phrase this well.. I just mean that since all ventilators come with a baseline controller, it is fair to build on top of that rather than just discard it.}\ug{Do we actually need this?}

% \paragraph{Deep Component.} On top of the baseline PID, we train a 2-layer neural network correction. The network takes as input a length $k=10$ history of previous errors $\{\epsilon_t \ldots \epsilon_{t-k}\}$, where $\epsilon_t := p^*_t - p_t$, thereby generalizing the class of linear error-feedback controllers (which contains PID). Our network first performs the following feature transformation
% \[ \left\{\epsilon'_i \defeq \frac{\sum_{j = 1}^{i} \epsilon_{t-j+1}}{i} \right\}_{i = 1 .. k},\]
% allowing it to react to the error feedback signal averaged over all time scales (further generalizing the PID controller). This is followed by a convolutional layer with kernel width $3$ and $5$ output channels and finally a fully connected layer.

% \paragraph{Training Specifics.} The deep component is trained via analytic policy gradient descent with the Adam optimizer \citep{kingma2017adam} leveraging automatic differentiation \emph{through the learned dynamics simulator(s)} with respect to the controller's parameters. Note that this is \emph{not} possible on a physical lung, and is a key advantage of our methodology. In the next section, we provide a comparison of popular zeroth-order policy gradient methods in terms of performance on the simulator and demonstrate the efficiency of this approach.  We detail our choice of hyperparameters in the Appendix.

\subsection{Experiments}

For our experiments, we use the physical test lung to run our proposed controllers (trained on the simulators) and compare it against the PID controller that perform best on the physical lung.

To make comparisons, we compute a score for each controller on a given test lung setting (e.g., $R=5, C=50$) by averaging the $L_1$ deviation from a target pressure waveform for all inspiratory phases, and then averaging these average $L_1$ errors over six waveforms specified in \citet{ISO68844}. We choose $L_1$ as an error metric so as not to over-penalize breaths that fall short of their target pressures and to avoid engineering a new metric. We determine the best performing PID controller for a given setting by running exhaustive grid searches over $P,I,D$ coefficients for each lung setting (details for both our score and the grid searches can be found in the Appendix).

% \paragraph{Tracking improvement.} For a given test lung setting, we compare the best performing PID controller for that setting to the controller trained using the simulator for that lung setting. For example, for $R=5, C=50$, we find the PID controller that performs best and compare it to our proposed controller trained on the simulator for $R=5, C=50$. We make this comparison on $R=\{5,20\} \times C=\{10, 20, 50\}$.

% \paragraph{Generalization.} For a \emph{set} of test lung settings, we compare the PID controller with the highest average score over that set of lung settings to a controller that was trained on the simulators corresponding to the same lung settings. We then evaluate performance for both controllers on each lung in the set. We focus on the settings $R=20, C=[10, 20, 50]$ since this set is the most commonly seen during the COVID-19 pandemic \citep{haudebourg2020respiratory}.

\begin{figure}[!h]
\centering 
\includegraphics[width=8cm]{figures/local.png}
\caption{We show that for each lung setting, the controller we trained on the simulator for that setting outperforms the best-performing PID controller found on the physical test lung.}\label{fig:results-tracking}
\end{figure}

% \paragraph{Numerical Results.}
% We benchmark the performance of the proposed controller in the graphs above. As shown in Figure~\ref{fig:results-tracking}, for the tracking improvement task, our separately-trained controllers outperform the best PID controllers tuned specifically to each lung setting. We improve upon the best PID for all lung settings where $R=5$ and $R=20$. For the generalization task over $R=20$ settings, we show that our proposed controller outperforms the best PID controller found over the three $R=20$ settings in each individual setting. What is more, our controller even outperforms the best PID controller in each setting as well.

\begin{figure}[!h]
\centering 
\includegraphics[width=8cm]{figures/global.png}
\caption{The controller we trained on all six simulators outperforms the best PID found over the the same six settings on the physical test lung. Of note, our wins are proportionally greater when trained on all six settings whereas individual lung settings are more achievable by PID alone.}\label{fig:results-generalization}
\end{figure}

\begin{figure}[!h]
\centering 
\includegraphics[width=8cm]{figures/traj-compare.pdf}
\caption{As an example, we compare our method (learned controller on learned simulator) to the best P-only, I-only, and PID controllers relative to a target waveform (dotted line). Whereas our controller rises quickly and stays very near the target waveform, the other controllers take significantly longer to rise, overshoot, and, in the case of P-only and PID, ring the entire inspiratory phase.}\label{fig:traj}
\end{figure}

% \paragraph{Qualitative Behavior.} In Figure~\ref{fig:traj}, we can see that the PID controller (orange) is insufficiently expressive to match the target waveform, undershooting the target waveform (dotted line) for most of the breath before overshooting, while ringing the entire time. By contrast, our controller rises quickly to the target pressure and maintains an even pressure for the majority of the inspiratory phase.


\section{Comparison of RL methods} \label{sec:benchmarks}
As part of our investigation, we benchmarked and compared several Reinforcement Learning(RL) methods for policy optimization on the simulator before settling on the analytic policy gradient approach that leverages the ability to differentiate through the simulated dynamics outlined before. We consider popular RL algorithms, namely PPO~\citep{ppo} and DQN~\citep{dqn} and compare them to direct analytical policy gradient descent. These algorithms are representative of two mainstream RL paradigms, policy gradient and Q-learning, respectively. We performed experiments on simulators that represent lungs with different R,C parameters. The metric as earlier is the L1 distance between the target and achieved lung pressure per step. To ensure a fair model comparison, we used the same state featurization (as described in the previous section) for all algorithms and performed extensive hyperparameter search for our baselines during the training phase. Results are shown in Figure~\ref{fig:baselines}. Our algorithm achieves comparable scores to the baselines across all simulators.

Importantly, our analytical gradient based method achieves a comparable score relative to PPO/DQN in orders of magnitude less samples. This sample-efficiency property of our algorithm can be clearly observed from  (Figure~\ref{fig:samplecomplexity}). Our method converges within ~100 episodes of training, while the other methods require tens of thousands of episodes. Further, our algorithm has a stable training process, in contrast to the notable training instability for the baselines. Furthermore, our method is robust with respect to hyperparameter tuning, unlike the baselines, which require an extensive search over hyperparameters to achieve comparable performance. This extensive hyperparameter search required by the baselines is unfeasible for use in resource-constrained or online learning scenarios, which are typical use cases for these control systems. Specifically for the results provided here, we conducted 720 trials with different hyperparameter configuration for PPO and 180 trials for DQN. In contrast, using our method only involves a few trials of standard optimizer learning rate tuning, which is the minimum effort in deep learning practices.

\begin{figure}[!h]
\centering 
\includegraphics[width=8cm]{ML4H 2021/figures/2rowbar.pdf}
\caption{Performance comparison of our controller with PPO/DQN. The score is calculated by average per-step L1 distance between target and achieved pressure.}\label{fig:baselines}
\end{figure}

\begin{figure}[!h]
\centering 
\includegraphics[width=8cm]{ML4H 2021/figures/samplecomplexity.pdf}
\caption{Convergence behavior demonstration. }\label{fig:samplecomplexity}
\end{figure}

==> ML4H 2021/7.conclusions.tex <==
\section{Conclusions and future work} \label{sec:discussion}

We have presented a machine learning approach to ventilator control, demonstrating the potential of end-to-end learned controllers by obtaining improvements over industry-standard baselines.
Our main conclusions are
\begin{enumerate}
    \item The nonlinear dynamical system of lung-ventilator can be modeled by a neural network more accurately than previously studied physics-based models.
    
    \item Controllers based on deep neural networks can outperform PID controllers across multiple clinical settings (waveforms), and can generalize better across patient lungs characteristics, despite having significantly more parameters. 
    
    \item 
    Direct policy optimization for differentiable environments has potential to significantly outperform Q-learning or (standard) policy gradient methods in terms of sample and computational complexity. 
    
\end{enumerate}

There remain a number of areas to explore, mostly motivated by medical need. The lung settings we examined are by no means representative of all lung characteristics (e.g., neonatal, child, non-sedated) and lung characteristics are not static over time; a patient may improve or worsen, or begin coughing. Ventilator costs also drive further research. As an example, inexpensive valves have less consistent behavior and longer reaction times, which exacerbate bad PID behavior (e.g., overshooting, ringing), yet are crucial to bringing down costs and expanding access. Learned controllers that adapt to these deficiencies may obviate the need for such trade-offs.

% As part of our study we make our simulators and code available to the scientific community, to lower the entrance cost into this important medical application.

%In the future we intend to enhance this preliminary study and focus on generalization and robustness. Can deep controllers give rise to more robust controllers across different types of lungs? Can they cope with spontaneous patient breathing? 





==> ML4H 2021/defs.tex <==

\newcommand{\softmax}{\text{softmax}}
\newcommand{\CH}{\text{CH}}
\newcommand{\F}{\mathcal{F}}
%\newcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\DeclareMathOperator{\Tr}{Tr}
\definecolor{PrincetonOrange}{HTML}{ff8f00}

% change these macros to different names.
\newcommand*{\affaddr}[1]{#1} % No op here. Customize it for different styles.
\newcommand*{\affmark}[1][*]{\textsuperscript{#1}}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}


\def\ltil{{{\tilde{\ell}}}}
\def\btalpha{{\bm{\tilde{\alpha}}}}
\def\balpha{{\bm{\alpha}}}
\def\talpha{{\tilde{\alpha}}}
\def\btbeta{{\bm{\tilde{\beta}}}}
\def\bbeta{{\bm{\beta}}}
\def\tbeta{{\tilde{\beta}}}
\def\btgamma{{\bm{\tilde{\gamma}}}}
\def\bgamma{{\bm{\gamma}}}
\def\tgamma{{\tilde{\gamma}}}


\def\mL{{\mathcal L}}

\def\X{{\mathcal X}}
\def\H{{\mathcal H}}
\def\Y{{\mathcal Y}}
\def\W{{\mathcal W}}
\def\R{{\mathbb R}}


% notation here
\newcommand{\ftil}{\tilde{f}}

\def\hestinv{\tilde{\nabla}^{-2}}
\def\hest{\tilde{\nabla}^{2}}
\def\hessinv{\nabla^{-2}}
\def\hess{\nabla^2}
\def\grad{\nabla}


% notation

\newcommand{\re}{{\text{Re}}}
\newcommand{\B}{B}
%\newcommand{\R}{\mathcal{R}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\cE}{\mathcal{E}}
\renewcommand{\sp}{\mathrm{span}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\cor}{\mathrm{cor}}
\newcommand{\sign}{\text{ } \mathrm{sign}}


\newcommand{\bzero}{\ensuremath{\mathbf 0}}
\newcommand{\y}{\ensuremath{\mathbf y}}
\newcommand{\z}{\ensuremath{\mathbf z}}
\newcommand{\h}{\ensuremath{\mathbf h}}
\newcommand{\K}{\ensuremath{\mathcal K}}
\def\bb{\mathbf{b}}
%\def\bc{\mathbf{c}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\C{{\mathcal C}}

%\def\be{\mathbf{e}}
\def\etil{\tilde{\mathbf{e}}}
%\def\bk{\mathbf{k}}
\def\bu{\mathbf{u}}
\def\x{\mathbf{x}}
\def\y{\mathbf{y}}
\def\w{\mathbf{w}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}

\def\bw{\mathbf{w}}
%\def\ba{\mathbf{a}}
\def\bA{\mathbf{A}}
\def\bS{\mathbf{S}}
\def\bG{\mathbf{G}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bV{\mathbf{V}}
\def\bone{\mathbf{1}}

\def\regret{\mbox{{Regret}}}

\def\ytil{\tilde{{y}}}
\def\yhat{\hat{{y}}}
\def\what{\hat{{w}}}
\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}



% comments, etc
\newcommand{\ignore}[1]{}
% for emails
\newcommand{\email}[1]{\texttt{#1}}



% repeated theorems

\newenvironment{repthm}[2][]{%
  \def\theoremauxref{\cref{#2}}
  \begin{theoremaux}[#1]
}{%
  \end{theoremaux}
}



% bold serif
\DeclareMathAlphabet{\mathbfsf}{\encodingdefault}{\sfdefault}{bx}{n}

% operators
\DeclareMathOperator*{\err}{error}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\supp}{supp}
%\DeclareMathOperator*{\poly}{poly}
\let\Pr\relax
\DeclareMathOperator{\Pr}{\mathbb{P}}

% cases
\newcommand{\mycases}[4]{{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}}
\end{array}
\right. }}

\newcommand{\mythreecases}[6] {{
\left\{
\begin{array}{ll}
    {#1} & {\;\text{#2}} \\[1ex]
    {#3} & {\;\text{#4}} \\[1ex]
    {#5} & {\;\text{#6}}
\end{array}
\right. }}

% macros
\newcommand{\lr}[1]{\!\left(#1\right)\!}
\newcommand{\lrbig}[1]{\big(#1\big)}
\newcommand{\lrBig}[1]{\Big(#1\Big)}
\newcommand{\lrbra}[1]{\!\left[#1\right]\!}
\newcommand{\lrnorm}[1]{\left\|#1\right\|}
\newcommand{\lrset}[1]{\left\{#1\right\}}
\newcommand{\lrabs}[1]{\left|#1\right|}
%\newcommand{\set}[1]{\{#1\}}
\newcommand{\abs}[1]{|#1|}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\renewcommand{\t}[1]{\smash{\tilde{#1}}}
\newcommand{\wt}[1]{\smash{\widetilde{#1}}}
\newcommand{\wh}[1]{\smash{\widehat{#1}}}
\renewcommand{\O}{O}
%\renewcommand{\O}{\mathcal{O}}
\newcommand{\OO}[1]{\O\lr{#1}}
\newcommand{\tO}{\wt{\O}}
\newcommand{\tTheta}{\wt{\Theta}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}[1]{\E\lrbra{#1}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\tsum}{\sum\nolimits}
\newcommand{\trace}{\mathrm{tr}}
\newcommand{\ind}[1]{\mathbb{I}\!\lrset{#1}}
\newcommand{\non}{\nonumber}
\newcommand{\poly}{\mathrm{poly}}

% \newcommand{\tr}{^{\mathsmaller\top}}
\newcommand{\tr}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\st}{\star}
\renewcommand{\dag}{\dagger}

%\newcommand{\kl}[2]{\mathsf{D}_\mathrm{KL}(#1,#2)}
\newcommand{\tv}[2]{\mathsf{D}_{\mathrm{TV}}(#1,#2)}
\newcommand{\ent}{\mathsf{H}}
\newcommand{\info}{\mathsf{I}}

\newcommand{\reals}{\mathbb{R}}
\newcommand{\eps}{\varepsilon}
\newcommand{\ep}{\varepsilon}
%\newcommand{\eps}{\epsilon}
\newcommand{\sig}{\sigma}
\newcommand{\del}{\delta}
\newcommand{\Del}{\Delta}
\newcommand{\lam}{\lambda}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\thalf}{\tfrac{1}{2}}

\newcommand{\eqdef}{:=}
\newcommand{\eq}{~=~}
\renewcommand{\leq}{~\le~}
\renewcommand{\geq}{~\ge~}
\newcommand{\lt}{~<~}
\newcommand{\gt}{~>~}
\newcommand{\then}{\quad\Rightarrow\quad}

\let\oldtfrac\tfrac
\renewcommand{\tfrac}[2]{\smash{\oldtfrac{#1}{#2}}}


\let\nablaold\nabla
\renewcommand{\nabla}{\nablaold\mkern-2.5mu}
%\let\cdotold\cdot
%\renewcommand{\cdot}{\mkern-2.5mu\cdotold\mkern-2.5mu}
%\newcommand{\param}{\cdotold}


%\newcommand{\diag}{\mathrm{diag}}
\newcommand{\nf}[2]{\nicefrac{#1}{#2}}
\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}
\newcommand{\ten}[1]{\mathcal{#1}}
\newcommand{\frob}[1]{\|#1\|_2}
\newcommand{\p}[2]{\textrm{Pr}[ #1\in #2] }
\newcommand{\pe}[2]{\mathop{\textrm{Pr}}\limits_{#1}\left[#2\right] }
%\newcommand{\one}[1]{\mathds{1}[#1]}
\newcommand{\inp}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\beps}{\bm{\eps}}
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\RE}[3]{\E{#1}{\sup_{#2}#3}}
%\newcommand{\rc}[1]{R\left(#1\right)}


==> ML4H 2021/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

